PUSH: a primal heuristic based on Feasibility PUmp and SHifting

This work describes PUSH, a primal heuristic combining Feasibility Pump and Shifting. The main idea is to replace the rounding phase of the Feasibility Pump with a suitable adaptation of the Shifting and other rounding heuristics. The algorithm presents different strategies, depending on the nature of the partial rounding obtained. In particular, we distinguish when the partial solution is feasible, infeasible with potential candidates, and infeasible without candidates. We used a threshold to indicate the percentage of variables to round with our algorithm and which other to round to the nearest integer. Most importantly, our algorithm tackles directly equality constraints without duplicating rows. We select the parameters of our algorithm on the 19 instances provided for the Mip Competition 2022. Finally, we compared our approach to other start heuristics, like Simple Rounding, Rounding, Shifting, and Feasibility Pump on the first 800 MIPLIB2017 instances ordered by the number of non-zeros.

==> introduction.tex <==
Primal heuristics are a fundamental  tool in optimization methods. They may be used by themselves to find quick feasible solutions, or they may be adopted as a part of exhaustive search algorithms. For this reason, during the years several strategies have been proposed, spanning from binary to mixed prblems, from linear to non-linear ones.

In this work, we will focus on Mixed Integer Linear Programs (MIP), which are a sub class of integer programming where the mathematical problem to be solved presents integer and continuous variables, but the relations among them in the objective and in constraints are all affine.

Among all the difference approaches, a big division can be made between start and improvement methods. The firsts focusing on finding a starting feasible solution, the seconds on improving a known one. 
A lot of rounding methods belong to the first group, like the Simple Rounding \cite{balas1980pivot}, 



Improvement heuristics try to improve a solution from a given feasible one; example of improvement heuristics are Local Branching \cite{fischetti2003local}, RINS (relaxation induced neighborhood search) \cite{danna2005exploring}, evolutionary algorithms \cite{rothberg2007evolutionary} and Dins \cite{ghosh2007dins}. 


In literature many heuristics have been proposed to find a solution of a Mixed-Integer-Program (MIP). This task is an NP-hard problem \cite{schrijver2003combinatorial} and so an high interest has been arose in developing fast methods to find a good solution in a low computational time. Particularly there are two main classes of heuristics that try to reach this goal: improvement heuristics and start heuristics.




Vice-versa start heuristics try to find a feasible solution of the MIP without knowing anything except for the structure of the problem. To build a feasible solution for the MIP these heuristics generally start from a solution obtained from the relaxation of the MIP and try to round fractional variables while maintaining LP feasibility (they are the so called rounding methods). An example of these is Rens \cite{berthold2007rens}. In this algorithm LP are solved iteratively until an integer solution is found: at each iteration the lower and upper bounds of fractional variables are changed. Quite good popularity reached rounding methods that use pivot and shifting; they are based on pivot operations (pivot) and how to round the fractional or continuous variables in a smart way (shifting). 
The first one of these heuristics was implemented by \cite{balas1980pivot} however developed just for Binary programs. In \cite{balas1986pivot} the algorithm was extended even to general MIP and was improved in \cite{balas2004pivot}. Another pivot heuristic is \cite{eckstein2007pivot} just for 0-1 Integer programs that exploit pivot operations, cuts and diving heuristics.

Another heuristic that solves iteratively LP is feasibility pump first introduced by \cite{fischetti2005feasibility} then it was generalized even to Mixed Integer Problems by \cite{bertacco2005feasibility}, \cite{achterberg2007improving} and improved by \cite{fischetti2009feasibility}, \cite{baena2010using} and \cite{boland2014boosting}.
Even the very popular Tabu Search \cite{glover1997tabu} was exploited to solve a 0-1 MIP by \cite{lokketangen1998solving}.
Instead an heuristic very different from the others and based essentially on geometrical ideas is Octane \cite{balas2001octane}.
 Obviously this is not an overall study of all MIP heuristics; however for a more comprehensive one you could refer to \cite{fischetti2010heuristics}-\cite{hanafi2017mathematical} . 






 Mixed Integer Problems (MIP)
